Tractable Dendritic RNNs for Reconstructing Nonlinear Dynamical Systems

In many scientific disciplines, we are interested in inferring the nonlinear dynamical system underlying a set of observed time series, a challenging task in the face of chaotic behavior and noise. Previous deep learning approaches toward this goal often suffered from a lack of interpretability and tractability. In particular, the high-dimensional latent spaces often required for a faithful embedding, even when the underlying dynamics lives on a lower-dimensional manifold, can hamper theoretical analysis. Motivated by the emerging principles of dendritic computation, we augment a dynamically interpretable and mathematically tractable piecewise-linear (PL) recurrent neural network (RNN) by a linear spline basis expansion. We show that this approach retains all the theoretically appealing properties of the simple PLRNN, yet boosts its capacity for approximating arbitrary nonlinear dynamical systems in comparatively low dimensions. We employ two frameworks for training the system, one combining back-propagation-through-time (BPTT) with teacher forcing, and another based on fast and scalable variational inference. We show that the dendritically expanded PLRNN achieves better reconstructions with fewer parameters and dimensions on various dynamical systems benchmarks and compares favorably to other methods, while retaining a tractable and interpretable structure.

==> figures/texfiles/3_bases_illustration.tex <==
\begin{figure}[!htp]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/images/explain/Figure1.jpg}
    \caption{Inspired by principles of dendritic computation, our \ourmethodname\ extends each unit into a set of nonlinear branches connected to a soma, yielding single unit transfer functions with increased approximation capabilities. Image of dendrite from \url{https://www.milad.no/blog/} (CC BY-SA 4.0).}
    % 
    
    %\caption{Inspired by dendritic computation, the proposed basis expansion compresses recurrent links $\alpha_1, \alpha_2, \alpha_3$ into an activation function.} 
    % Milad Mobarhan image source website: https://www.milad.no/blog/
    \label{fig:base_illustration}
\end{figure}

% Figure 2. Examples of low-dimensional model reconstructions: (a) Time series (left) and state space trajectories (right) for the original Lorenz-63 chaotic attractor and simulations produced by a trained spline-PLRNN (B=***, M=***, tau=***). (b) Same for a bursting neuron model (hyper-parameters of spline-PLRNN: B=***, M=***, tau=***). 

% Figure 3. Examples of high-dimensional model reconstructions: (a) Time series (left), spatio-temporal evolution (center), and power spectra (right) for the true 10d Lorenz-96 system and for spline-PLRNN simulations (B=***, M=***, tau=***). (b) Same for a 50d neural population model producing coherent chaos (hyper-parameters of spline-PLRNN: B=***, M=***, tau=***).

% Figure 4. Effect of basis expansion for Lorenz-63 and Lorenz-96 systems. (a) 25-step ahead prediction error (left) and agreement in attractor geometries (right) as a function of the number of bases ($B$) for fixed numbers of total parameters. (b) 25-step ahead prediction error (left) and agreement in attractor geometries (right) as a function of the number of bases ($B$) for different numbers of latent states ($M$). Horizontal lines indicate iso-performance levels.

% Figure 5. Dimensionality reduction through basis expansion for low-dimensional Lorenz-63 (a, b) and high-dimensional Lorenz-96 (c, d) systems.

==> figures/texfiles/4_1_1_examples_low_dimensional_systems.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=1.\linewidth]{figures/images/examples/low_all_flo.PNG}  
\caption{Examples of low-dimensional model reconstructions: (a) Time series (left) and state space trajectories (right) for the original Lorenz-63 chaotic attractor and simulations produced by a \ourmethodname\ trained with VI ($B=20$, $M=15$, $\lambda=1$, $M_{\textrm{reg}}/M=0.5$). Dots indicate true and reconstructed fixed points. (b) Same for the bursting neuron model, produced by a \ourmethodname\ trained with TF ($B=47$, $M=26$, $\tau=5$). Note that the bursting is a complex limit cycle but \textit{non-chaotic}.}
\label{fig:low_dim_examples}
\end{figure}

% \begin{figure}[ht]

% \begin{subfigure}{.48\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/images/examples/low_lorenz.pdf}  
%   \caption{}
%   \label{fig:sub-first}
% \end{subfigure}
% \begin{subfigure}{.48\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/images/examples/low_burstingneuron.pdf}  
%   \caption{}
%   \label{fig:sub-second}
% \end{subfigure}

% \label{fig:fig}
% \caption{Examples of low-dimensional model reconstructions: (a) Time series (left) and state space trajectories (right) for the original Lorenz-63 chaotic attractor and simulations produced by a trained \ourmethodname\ ($B=20$, $M=15$, $\tau=1$). Dots indicate true and reconstructed fixed points. (b) Same for a bursting neuron model (hyper-parameters of \ourmethodname\: $B=50$, $M=15$, $\tau=1.5$).}
% \end{figure}



==> figures/texfiles/4_1_2_examples_high_dim_systems.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=.75\linewidth]{figures/images/examples/high_all.jpg}  
\caption{Examples of high-dimensional model reconstructions: (a) Time series (left), spatio-temporal evolution (center), and power spectra (right) for the true 10d Lorenz-96 system and for \ourmethodname\ simulations ($B=50$, $M=30$, $\lambda=1.0$, $M_{\textrm{reg}}/M=1.0$). (b) Same for a 50d neural population model producing coherent chaos ($B=5$, $M=12$, $\lambda=1.0$, $M_{\textrm{reg}}/M=0.2$).}
\label{fig:high_dim_examples}
\end{figure}

% \begin{figure}[ht]

% \begin{subfigure}{1.\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/images/examples/high_l96.pdf}  
%   \caption{}
%   \label{fig:sub-first}
% \end{subfigure}
% \begin{subfigure}{1.\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/images/examples/high_cc.pdf}  
%   \caption{}
%   \label{fig:sub-second}
% \end{subfigure}

% \label{fig:fig}
% \caption{Examples of high-dimensional model reconstructions: (a) Time series (left), power spectra (center), and spatio-temporal evolution (right) for the true 10d Lorenz-96 system and for \ourmethodname\ simulations ($B=50$, $M=30$, $\tau=1$). (b) Same for a 50d neural population model producing coherent chaos (hyper-parameters of \ourmethodname\: $B=5$, $M=12$, $\tau=1$).}
% \end{figure}



% \begin{figure}[ht]

% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/images/examples/high_l96_traj.pdf} 
%   \caption{}
%   \label{fig:sub-first}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/images/examples/high_l96_ps.pdf}  
%   \caption{}
%   \label{fig:sub-second}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/images/examples/high_l96_pattern.pdf}
%   \caption{}
%   \label{fig:sub-second}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/images/examples/high_cc_traj.pdf}
%   \caption{}
%   \label{fig:sub-first}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/images/examples/high_cc_ps.pdf}
%   \caption{}
%   \label{fig:sub-second}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/images/examples/high_cc_pattern.pdf}  
%   \caption{}
%   \label{fig:sub-second}
% \end{subfigure}
% \caption{Examples of high-dimensional model reconstructions: (a) Time series (left), power spectra (center), and spatio-temporal evolution (right) for the true 10d Lorenz-96 system and for \ourmethodname\ simulations ($B=50$, $M=30$, $\tau=1$). (b) Same for a 50d neural population model producing coherent chaos (hyper-parameters of \ourmethodname\: $B=5$, $M=12$, $\tau=1$).}
% \label{fig:fig}
% \end{figure}

==> figures/texfiles/4_figure4.tex <==
\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{figures/images/parcontrol/Figure4a.PNG}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{figures/images/parcontrol/Figure4b.PNG}
\end{subfigure}
\caption{Effect of basis expansion for dendPLRNN trained by VI. (a)  Agreement in attractor geometries (left) and 20-step ahead prediction error (right) for the Lorenz-63 system as a function of the number of bases ($B$) for fixed numbers of total parameters. (b)  Agreement in attractor geometries (left) and 20-step ahead prediction error (right) for the Lorenz-63 system as a function of the number of bases ($B$) for different numbers of latent states ($M$). %, with the black dots marking the achievable dimensionality reduction with different $B$.
}
\label{fig:effect_basis_expansion}
\end{figure}

==> figures/texfiles/6_EEG.tex <==
\begin{figure}[!htb]
    \centering
	\includegraphics[width=0.99\linewidth]{figures/images/supplements/EEG_overview}
	\caption{EEG recordings from frontal, occipital, parietal and temporal lobe vs. freely generated trajectories, sampled from the \ourmethodname, trained with BPTT ($M=128, B=50, \tau=10, M_{\textrm{reg}}/M=0.5, \lambda=1.0$).}

	\label{fig:EEG_trajectory}
\end{figure}

==> figures/texfiles/6_klx_correlation.tex <==
\begin{figure}[!htb]
    \centering
	\includegraphics[width=0.5\linewidth]{figures/images/supplements/6_dstps_corr.PNG}
	\caption{Correlation between the binning approximation ($m=30$)  %($D_{\text{stsp}}$)
	and the logarithm of the GMM approximation ($\sigma^2=1$) to $D_{stsp}$ on the Lorenz-63 system for different noise realizations and variances. Similar as reported for the $KL_\bold{Z}$ approximation in \cite{koppe_identifying_2019} we observed a logarithmic relation between the GMM and binning based measures.
	%To obtain this figure, a dataset derived from a Lorenz system was increasingly distorted by noise, and agreement between ground truth data and the distorted dataset was computed for both methods.
	}
	\label{fig:klx_correlation}
\end{figure}

==> figures/texfiles/6_lorenz_fixedpoints.tex <==
\begin{figure}[!htb]
    \centering
	\includegraphics[width=0.5\linewidth]{figures/images/lorenz/lorenz_fixedpoint_withTrue.pdf}
	\caption{3 Unstable fixed points obtained from a successfully reconstructed Lorenz system (red) and ground-truth (also unstable) fixed points (green).}

	\label{fig:lorenz_attractor-fp}
\end{figure}

==> figures/texfiles/6_parcontrol.tex <==
\begin{figure}[!htb]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{figures/images/parcontrol/6a_bursting_params.PNG}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{figures/images/parcontrol/6b_lorenz96_statebase.PNG}
\end{subfigure}
\caption{Effect of basis expansion for dendPLRNN trained by VI. (a)  Agreement in attractor geometries (left) and 20-step ahead prediction error (right) for the bursting neuron system as a function of the number of bases ($B$) for fixed numbers of total parameters. (b)  Agreement in power spectrum correlation (left) and 20-step ahead prediction error (right) for the Lorenz-96 system as a function of the number of bases ($B$) for different numbers of latent states ($M$). %, with the black dots marking the achievable dimensionality reduction with different $B$.
}
\label{fig:supp:parcontrol}
\end{figure}

==> files/7_acknowledgements.tex <==
This work was funded by the German Research Foundation (DFG) within Germany’s Excellence Strategy – EXC-2181 – 390900948 (’Structures’), by DFG grant Du354/10-1 to DD, and the European Union Horizon-2020 consortium SC1-DTH-13-2020 ('IMMERSE').

==> files/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    Yes. % maybe spell out our claims and in which way we address them
  \item Did you describe the limitations of your work?
    Yes, in the conclusion.
  \item Did you discuss any potential negative societal impacts of your work?
    Yes, in the conclusion.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    Yes.
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    Yes. 
	\item Did you include complete proofs of all theoretical results?
    Yes, in the supplementary materials we included a proof for every proposition in the main text.
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    We included the code base in the supplementary material (to maintain anonymity), but will publish it after the publication.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    Yes, details are in the supplementary material.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    Yes.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    Yes, we referenced in Sec. \ref{sec:experiments}, that we used an internal cluster with 100 CPU cores. One setting (in total 1600 runs of our algorithm) e.g. for Fig. \ref{fig:effect_basis_expansion} distributed among these cores takes about 24 hours to compute.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    Yes, we cited Pathak et al. \cite{pathak_model-free_2018}, Vlachas et al. \cite{vlachas_backpropagation_2020} and Brunton et al. \cite{brunton_discovering_2016} in the experimental section at the appropriate places.
  \item Did you mention the license of the assets?
    Yes. For Fig. \ref{fig:base_illustration} we used an image with CC BY-SA 4.0 (as mentioned in the caption).
  \item Did you include any new assets either in the supplemental material or as a URL?
    Yes.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    Not applicable. The image was licensed under CC BY-SA 4.0, and for the academic work we cited the sources.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    Not applicable.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    Not applicable.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    Not applicable.
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    Not applicable.
\end{enumerate}

\end{enumerate}
